Regular Seifert surfaces and Vassiliev knot invariants

We show that the Vassiliev invariants of orders $\leq n$ of a knot K, are obstructions to finding a regular Seifert surface, S, whose complement looks "simple" (e.g. like the complement of a disc) to the lower central series of its fundamental group. As a consequence of this, we obtain that the Vassiliev invariants of the knot $K=\partial S$ are null-concordance obstructions of certain links that can be obtained from regular spines of S. We also discuss various generalizations of these results, and we conjecture a geometric characterization of knots whose invariants of all orders vanish.

==> ntmacros.tex <==
\magnification=1200
\catcode`\@=11

\font\tenmsx=msam10
\font\sevenmsx=msam7
\font\fivemsx=msam5
\font\tenmsy=msbm10
\font\sevenmsy=msbm7
\font\fivemsy=msbm5
%\font\fivemsbm=msbm5
%\font\sevenmsbm=msbm7
\font\B=cmbx8 at 8pt
\font\BC=cmbx9 at 9pt
\newfam\msxfam
\newfam\msyfam
%\newfam\msbmfam
\textfont\msxfam=\tenmsx  \scriptfont\msxfam=\sevenmsx
  \scriptscriptfont\msxfam=\fivemsx
\textfont\msyfam=\tenmsy  \scriptfont\msyfam=\sevenmsy
\scriptscriptfont\msyfam=\fivemsy
%\textfont\msbmfam=\sevenmsbm \scriptfont\msbmfam=\fivemsbm

\def\Bbb{\ifmmode\let\next\Bbb@\else
 \def\next{\errmessage{Use \string\Bbb\space only in math mode}}\fi\next}
\def\Bbb@#1{{\Bbb@@{#1}}}
\def\Bbb@@#1{\fam\msyfam#1}

\baselineskip=15pt
%\footline={\tenrm  \phantom{a} \folio}
%\nopagenumbers
%\baselineskip=13pt
\font\small=cmr9 at 9pt
%\bffont\b=cmr9 at 9pt
\font\Small=cmr7 at 7pt
\font\Smaller=cmr6 at 6pt
%\font\skata=cmr15 at 15pt
\font\msmall=cmr8 at 8pt
\font\vsmall=cmsl9 at 9pt
\font\mi=cmmi8 at 8pt
\font\i=cmti9 at 9pt
\font\B=cmr8 at 8pt
\font\BC=cmbx9 at 9pt

\def\Z{{\Bbb Z}}
\def\Q{{\Bbb Q}}
\def\N{{\Bbb N}}
\def\R{{\Bbb R}}


\overfullrule=0.0pt
\hsize=5.9truein
\vsize=8.45truein
\hoffset=.38truein
\voffset=.45truein
\def\p{\noindent}
\def\qed {\nobreak$\quad$\lower 1pt\vbox{
    \hrule
    \hbox to 6pt{\vrule height 6pt\hfil\vrule height 6pt}
      \hrule}\ifmmode\relax\else\par\medbreak \fi}





